Augmenting Modelers with Semantic Autocompletion of Processes

Business process modelers need to have expertise and knowledge of the domain that may not always be available to them. Therefore, they may benefit from tools that mine collections of existing processes and recommend element(s) to be added to a new process that they are constructing. In this paper, we present a method for process autocompletion at design time, that is based on the semantic similarity of sub-processes. By converting sub-processes to textual paragraphs and encoding them as numerical vectors, we can find semantically similar ones, and thereafter recommend the next element. To achieve this, we leverage a state-of-the-art technique for embedding natural language as vectors. We evaluate our approach on open source and proprietary datasets and show that our technique is accurate for processes in various domains.

==> performance.tex <==
\subsection{Performance}
We stress tested our system to evaluate how fast it can make the prediction and how scaleable our solution is. Our recommendation engine was running in docker container~\cite{docker}, with a flask service~\cite{flask} put in charge of serving the clients' requests. To simulate multiple users accessing the engine, we used an open source load testing tool called Locust~\cite{locust}. This tool allowed us to stress test the REST API that was provided via the flask service. Each request made to that service contained a workflow, specified in a BPMN format, an identification of the task for which the recommendations were made and a user identifier. The result of the REST API call was a list of predictions, including the recommended task name and type and also some additional textual information used for explaining the predictions to the user. 

In two different executions, we simulated $10$ and $100$ users concurrently accessing the recommendation engines. Each request was issued after a wait time uniformly distributed between $1$ and $5$ seconds. We used two different workflows for making the prediction. One was a small workflow with $5$ nodes and another one was a larger workflow with $25$ nodes. We also simulated two execution modes. One that was using gateways for prediction and another that was only looking at tasks. Thus, we had four different request types from which the stress test selected one type at random before issuing the request. 
For each configuration we let the stress test run until $10K$ requests have been completed. The results are shown in Table~\ref{tbl:perf}.

The average time it takes to recommend the next task varies between $308$ (for $10$ users) and $640$ milliseconds (for $100$ users). The $90\textsuperscript{th}$ percentile is under $1$ second in both cases and the maximum reaches $1641$. From the end user's perspective, in more than $90\%$ of the cases the wait time will be less than $1$ second, which is acceptable. For the remaining $10\%$ of the cases, the wait time is under $2$ seconds. In these cases the end user might decide skip the recommendation step. 
There were $4$ requests (out of $10K$) that resulted in an error returned from the server. In such a scenario, no recommendation are presented to the end user. 

\setlength{\tabcolsep}{6pt}
\begin{table}
	\centering
	\scriptsize
		\renewcommand\arraystretch{1.3}
		
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{\#Users}  &  Avg &  \multicolumn{4}{c|}{ Response Time (ms)} & \multirow{2}{*}{Failures}  
			  \tabularnewline
		\cline{3-6}
		 &  \#Reqs/sec & Avg  & Min & Max & 90\textsuperscript{th} perc. &
			  \tabularnewline
		\hline\hline
		10 & 3 & 308 & 203 & 907 & 390 & 0\% 
			\tabularnewline
		\hline
		100 & 30 & 640 & 206 & 1641 & 970 & 0.04\% 
			\tabularnewline
		\hline
	\end{tabular}
	\vspace{0.2cm}
	\caption{Performance measurements.}
	\label{tbl:perf}
\end{table}
